EMPRESS. II. Highly Fe-Enriched Metal-poor Galaxies with $\sim 1.0$ (Fe/O)$_\odot$ and $0.02$ (O/H)$_\odot$ : Possible Traces of Super Massive ($>300 M_{\odot}$) Stars in Early Galaxies

We present element abundance ratios and ionizing radiation of local young low-mass (~$10^{6}$ M_sun) extremely metal poor galaxies (EMPGs) with a 2% solar oxygen abundance (O/H)_sun and a high specific star-formation rate (sSFR~300 Gyr$^{-1}$), and other (extremely) metal poor galaxies, which are compiled from Extremely Metal-Poor Representatives Explored by the Subaru Survey (EMPRESS) and the literature. Weak emission lines such as [FeIII]4658 and HeII4686 are detected in very deep optical spectra of the EMPGs taken with 8m-class telescopes including Keck and Subaru (Kojima et al. 2019, Izotov et al. 2018), enabling us to derive element abundance ratios with photoionization models. We find that neon- and argon-to-oxygen ratios are comparable to those of known local dwarf galaxies, and that the nitrogen-to-oxygen abundance ratios (N/O) are lower than 20% (N/O)_sun consistent with the low oxygen abundance. However, the iron-to-oxygen abundance ratios (Fe/O) of the EMPGs are generally high; the EMPGs with the 2%-solar oxygen abundance show high Fe/O ratios of ~90-140% (Fe/O)_sun, which are unlikely explained by suggested scenarios of Type Ia supernova iron productions, iron's dust depletion, and metal-poor gas inflow onto previously metal-riched galaxies with solar abundances. Moreover, these EMPGs have very high HeII4686/H$\beta$ ratios of ~1/40, which are not reproduced by existing models of high-mass X-ray binaries whose progenitor stellar masses are less than 120 M_sun. Comparing stellar-nucleosynthesis and photoionization models with a comprehensive sample of EMPGs identified by this and previous EMPG studies, we propose that both the high Fe/O ratios and the high HeII4686/H$\beta$ ratios are explained by the past existence of super massive ($>$300 M_sun) stars, which may evolve into intermediate-mass black holes ($\gtrsim$100 M_sun).

==> ion_temperature.tex <==
\begin{table}[!hbtp]
\caption{Electron Temperature Adopted in the Ionic Abundance Estimation}
\begin{center}
\scriptsize{
\begin{tabular}{ccc}
\hline\noalign{\vskip3pt} 
Ion &
Ionization Potential &
Temperature  \\ 
 &
 (eV) &
 \\ 
(1)  &
(2) &
(3) \\ \hline\hline
O$^{2+}$ & %%%%%
35.1 &
$T_{\mathrm e}$({\sc{Oiii}})  \\
Ne$^{2+}$ & %%%%%
41.0 &
$T_{\mathrm e}$({\sc{Oiii}})  \\
Ar$^{3+}$ & %%%%%
40.7 &
$T_{\mathrm e}$({\sc{Oiii}})  \\ \hline
Ar$^{2+}$ & %%%%%
27.6 &
$T_{\mathrm e}$({\sc{Siii}})  \\ \hline
O$^{+}$ & %%%%%
13.6 &
$T_{\mathrm e}$({\sc{Oii}})  \\
N$^{+}$ & %%%%%
13.6 &
$T_{\mathrm e}$({\sc{Oii}})  \\
Fe$^{2+}$ & %%%%%
16.2 &
$T_{\mathrm e}$({\sc{Oii}})  \\
\hline\noalign{\vskip3pt} 
\end{tabular}}
\end{center}
{\footnotesize 
(1) Ions.
(2) Ionization potentials needed to produce the corresponding ions.
(3) Type of electron temperature adopted in the ionic abundance estimation. 
}\label{tbl:ion_temp}
\end{table}

